Protograph-Based LDPC Code Design for Ternary Message Passing Decoding

A ternary message passing (TMP) decoding algorithm for low-density parity-check codes is developed. All messages exchanged between variable and check nodes have a ternary alphabet, and the variable nodes exploit soft information from the channel. A density evolution analysis is developed for unstructured and protograph-based ensembles. For unstructured ensembles the stability condition is derived. Optimized ensembles for TMP decoding show asymptotic gains of up to 0.6 dB with respect to ensembles optimized for binary message passing decoding. Finite length simulations of codes from TMP-optimized ensembles show gains of up to 0.5 dB under TMP compared to protograph-based codes designed for unquantized belief propagation decoding.

==> figures/growthrate_2.tex <==
\begin{tikzpicture}





\node(img1){\input{figures/growthrate.tex}};
\node(img2)at(img1.south east)[yshift=3.5cm] [xshift=-1cm]  {	\input{figures/zoom.tex} };


\end{tikzpicture}%

==> figures/zoom.tex <==
\begin{tikzpicture}
\footnotesize

\begin{axis}
[
width=4.5cm,
height=3cm,
xmin=0,
xmax=0.008,
ymin=-0.005,
ymax=0.005,
ytick={-0.005,0,0.005},
]
\footnotesize
\addplot[line width=1,TUMBeamerRed,mark=none, mark options={solid}]
table[x=omega ,y=G,col sep=space,trim cells=true] {data/growthrate4_5zoom.txt};


\addplot[line width=1,color = black,dashed,mark=none, mark options={solid}]
	table[x=omega,y=G,col sep=space,trim cells=true] {data/line0.txt};
	
\addplot[line width=1,TUMBeamerOrange, only marks,mark = star,mark options={scale=1}]
table[x=omega ,y=G,col sep=space,trim cells=true] {data/omegastar.txt};

%\addplot[line width=1,TUMBeamerGreen,mark=none, mark options={solid}]
%table[x=omega ,y=G,col sep=space,trim cells=true] {data/growthraterandom4_5.txt};

\addplot[line width=1,TUMBeamerBlue,mark=none, mark options={solid}]
table[x=omega ,y=G,col sep=space,trim cells=true] {data/growthrateARJA4_5.txt};

\addplot[line width=1,cyan, only marks,mark = star,mark options={scale=1}]
table[x=omega ,y=G,col sep=space,trim cells=true] {data/omegastarARJA.txt};
	\end{axis}
\end{tikzpicture}%
